DoubleCheck: Designing Community-based Assessability for Historical Person Identification

Historical photos are valuable for their cultural and economic significance, but can be difficult to identify accurately due to various challenges such as low-quality images, lack of corroborating evidence, and limited research resources. Misidentified photos can have significant negative consequences, including lost economic value, incorrect historical records, and the spread of misinformation that can lead to perpetuating conspiracy theories. To accurately assess the credibility of a photo identification (ID), it may be necessary to conduct investigative research, use domain knowledge, and consult experts. In this paper, we introduce DoubleCheck, a quality assessment framework for verifying historical photo IDs on Civil War Photo Sleuth (CWPS), a popular online platform for identifying American Civil War-era photos using facial recognition and crowdsourcing. DoubleCheck focuses on improving CWPS's user experience and system architecture to display information useful for assessing the quality of historical photo IDs on CWPS. In a mixed-methods evaluation of DoubleCheck, we found that users contributed a wide diversity of sources for photo IDs, which helped facilitate the community's assessment of these IDs through DoubleCheck's provenance visualizations. Further, DoubleCheck's quality assessment badges and visualizations supported users in making accurate assessments of photo IDs, even in cases involving ID conflicts.

==> sections/cwps.tex <==
\section{Appendix}

==> sections/interactiongoals.tex <==
\section{Interaction Goals}

\subsection{Goal 1: Allow users to distinguish between photo comparison and photo identification}

To avoid potential misidentifications resulting from mixing facial similarity with photo identification, users should have the option to make their decision in a structured manner, by first comparing the photos and then identifying. Users are more likely to make accurate identifications, if they are confident about both facial similarity and the biographical details aligning up. Furthermore, showing other users the underlying processes and decisions involved in the identification would help them in assessing the quality of the identification. 

\subsection{Goal 2: Capture and display fine-grained information about facial similarity}

Mohanty et al. \cite{} found that photos matched on CWPS can be broadly divided into two types of visual matches: a facial match (i.e., two different photos of the same person) and a replica (i.e., two different copies of the same photo). Prior work has shown face recognition to work better at identifying replicas than facial matches \cite{}. In general, human users will find it easier to analyze replicas compared to facial matches. Displaying information about the match type, and if it is supported by facial recognition and the community, can help users assess better whether the two photos show the same person or not. In other words, this will indicate the reliability of the matched photos as supporting evidence for the identification. Users should be able to specify the visual match type, and the community should also be able to weigh in on existing photo matches, expressing whether they agree or disagree with the matches. 


\subsection{Goal 3: Allow users to indicate their confidence about an identification}

Allowing users to indicate how confident they are about the identification can result in more accurate decision-making. Users should also have the option to rule out candidates. In addition to that, allowing them to provide a note describing their rationale can help strengthen their case. Further, this information about confidence levels and decision rationale can also help other users in making a more accurate assessment of the identifications.

\subsection{Goal 4: Capture and display comprehensive provenance information}

Users should be able to indicate whether they knew the identity of a photo prior to uploading or not, and if so, they should provide the source of the photo’s identity. Capturing and displaying more comprehensive provenance about the photo’s identity from the users can overall improve the quality of an identification, and also allow other users to assess the information better.

\subsection{Goal 5: Support community validation of photo identifications}

Prior work has shown that novice crowd workers can reduce false positives suggested by face recognition, and assist experts in person identification tasks \cite{}. The CWPS community comprises users from different backgrounds and expertise areas, but the "wisdom of crowds" is not fully leveraged for verifying identities or debunking misidentifications. Allowing the community to express and check diverse opinions over existing identities on CWPS can help both in improving and assessing the quality of an identification. 

\subsection{Goal 6: Indicate photo identification quality and source reliability}

Credibility indicators have proven to be effective in helping users assess the content on websites, search engines, and social media \cite{}. Extending this notion of quality indicators to CWPS can help users in assessing the quality of photo identifications, especially novice users. Further, historians may want to query the database using these indicators to retrieve only research-grade identifications. These indicators should be prominent and reflect 1) an accurate assessment of the identification by factoring in critical information such as provenance, and 2) the different stages of identity verification (i.e., whether it needs more evidence, or it is airtight). Indicating the quality of a photo identification can help users effectively assess the information. Further, displaying information about the reliability and trustworthiness of the different sources used for the identification can also help the users. 


